Revisiting Neuron Coverage Metrics and Quality of Deep Neural Networks

Deep neural networks (DNN) have been widely applied in modern life, including critical domains like autonomous driving, making it essential to ensure the reliability and robustness of DNN-powered systems. As an analogy to code coverage metrics for testing conventional software, researchers have proposed neuron coverage metrics and coverage-driven methods to generate DNN test cases. However, Yan et al. doubt the usefulness of existing coverage criteria in DNN testing. They show that a coverage-driven method is less effective than a gradient-based method in terms of both uncovering defects and improving model robustness. In this paper, we conduct a replication study of the work by Yan et al. and extend the experiments for deeper analysis. A larger model and a dataset of higher resolution images are included to examine the generalizability of the results. We also extend the experiments with more test case generation techniques and adjust the process of improving model robustness to be closer to the practical life cycle of DNN development. Our experiment results confirm the conclusion from Yan et al. that coverage-driven methods are less effective than gradient-based methods. Yan et al. find that using gradient-based methods to retrain cannot repair defects uncovered by coverage-driven methods. They attribute this to the fact that the two types of methods use different perturbation strategies: gradient-based methods perform differentiable transformations while coverage-driven methods can perform additional non-differentiable transformations. We test several hypotheses and further show that even coverage-driven methods are constrained only to perform differentiable transformations, the uncovered defects still cannot be repaired by adversarial training with gradient-based methods. Thus, defensive strategies for coverage-driven methods should be further studied.

==> Makefile <==
# Makefile for a latex paper
LATEX = TEXINPUTS=$(TEXINPUTS):packages pdflatex
PAPER = Coverage_metrics

all: $(PAPER).pdf

#I don't have gs and don't want to see errors
quick: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
$(PAPER).pdf: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null
	gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -dEmbedAllFonts=true \
       -dDownsampleColorImages=false -dAutoFilterColorImages=false \
       -dColorImageFilter=/FlateEncode -sDEVICE=pdfwrite -sOutputFile=$(PAPER)-embed.pdf \
       $(PAPER).pdf
	mv $(PAPER)-embed.pdf $(PAPER).pdf

Figures: 
	
.PHONY: pdf print
print: $(PAPER).pdf
	open $(PAPER).pdf

clean:
	rm -f *.aux *.log $(PAPER).pdf *.blg *.bbl *.lof *.lot *.toc *.fls *.out *.fdb_latexmk *.cut *~

